DRL4AOI: A DRL Framework for Semantic-aware AOI Segmentation in Location-Based Services

In Location-Based Services (LBS), such as food delivery, a fundamental task is segmenting Areas of Interest (AOIs), aiming at partitioning the urban geographical spaces into non-overlapping regions. Traditional AOI segmentation algorithms primarily rely on road networks to partition urban areas. While promising in modeling the geo-semantics, road network-based models overlooked the service-semantic goals (e.g., workload equality) in LBS service. In this paper, we point out that the AOI segmentation problem can be naturally formulated as a Markov Decision Process (MDP), which gradually chooses a nearby AOI for each grid in the current AOI's border. Based on the MDP, we present the first attempt to generalize Deep Reinforcement Learning (DRL) for AOI segmentation, leading to a novel DRL-based framework called DRL4AOI. The DRL4AOI framework introduces different service-semantic goals in a flexible way by treating them as rewards that guide the AOI generation. To evaluate the effectiveness of DRL4AOI, we develop and release an AOI segmentation system. We also present a representative implementation of DRL4AOI - TrajRL4AOI - for AOI segmentation in the logistics service. It introduces a Double Deep Q-learning Network (DDQN) to gradually optimize the AOI generation for two specific semantic goals: i) trajectory modularity, i.e., maximize tightness of the trajectory connections within an AOI and the sparsity of connections between AOIs, ii) matchness with the road network, i.e., maximizing the matchness between AOIs and the road network. Quantitative and qualitative experiments conducted on synthetic and real-world data demonstrate the effectiveness and superiority of our method. The code and system is publicly available at https://github.com/Kogler7/AoiOpt.

==> plots/hyper-parameters.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
d & 1 & 2 & 4 \\
32 & 83.745 & 80.928 & 73.386 \\
64 & 87.682 & 83.584 & 78.461 \\
128 & 89.071 & 84.373 & 80.828 \\
192 & 89.104 & 84.595 & 79.262 \\
256 & 89.625 & 84.595 & 80.218 \\
}\paramDPrec

\pgfplotstableread[row sep=\\,col sep=&]{
d & 1 & 2 & 4 \\
32 & 264.88 & 344.56 & 522.35 \\
64 & 166.39 & 224.82 & 341.8 \\
128 & 133.38 & 192.54 & 304.72 \\
192 & 128.43 & 185.23 & 309.36 \\
256 & 118.64 & 180.47 & 298.38 \\
}\paramDMAE

\pgfplotstableread[row sep=\\,col sep=&]{
N_h & 1 & 2 & 4 \\
1 & 87.089 & 82.233 & 77.846 \\
2 & 87.766 & 83.632 & 78.786 \\
4 & 88.401 & 84.361 & 80.023 \\
8 & 89.071 & 84.373 & 80.828 \\
16 & 88.94 & 84.082 & 79.256 \\
}\paramNhPrec

\pgfplotstableread[row sep=\\,col sep=&]{
N_h & 1 & 2 & 4 \\
1 & 144.53 & 238.42 & 378.61 \\
2 & 134.91 & 196.94 & 328.19 \\
4 & 148.86 & 206.03 & 333.69 \\
8 & 133.38 & 192.54 & 304.72 \\
16 & 130.59 & 189.37 & 300.77 \\
}\paramNhMAE

\pgfplotstableread[row sep=\\,col sep=&]{
delta & 1 & 2 & 4 \\
10 & 80.152 & 76.978 & 73.913 \\
50 & 87.024 & 82.681 & 78.256 \\
100 & 89.071 & 84.373 & 80.828 \\
150 & 88.907 & 83.487 & 79.729 \\
200 & 89.165 & 83.721 & 80.085 \\
}\paramDeltaPrec

\pgfplotstableread[row sep=\\,col sep=&]{
delta & 1 & 2 & 4 \\
10 & 122.82 & 175.87 & 306.2 \\
50 & 135.75 & 189.58 & 319.5 \\
100 & 133.38 & 192.54 & 304.72 \\
150 & 133.33 & 185.85 & 306.18 \\
200 & 136.73 & 191.83 & 304.78 \\
}\paramDeltaMAE

\resizebox{1.0\linewidth}{!}{
    \begin{tikzpicture}
    \begin{customlegend}[legend columns=3,legend style={align=center,column sep=1ex},
            legend entries={$\mu=1$ minute,$\mu=2$ minutes,$\mu=4$ minutes}]
            \addlegendimage{color=pt1min,mark=square*}
            \addlegendimage{color=pt2min,mark=triangle*}
            \addlegendimage{color=pt4min,mark=otimes*}
            \end{customlegend}
    \end{tikzpicture}
}

\tikzset{every plot/.style={line width=1.2pt}}

\subfigure[Embedding dimension $d$] {
    \resizebox{0.49\linewidth}{!}{
        \begin{tikzpicture}
        \begin{axis}[
            width=0.75\linewidth,
            ylabel={Precision (\%)},
            ymin=73, ymax=91,
            ytick distance={3},
            ymajorgrids=true,
            grid style=dashed,
            xtick=data,
            symbolic x coords={32,64,128,192,256},
            nodes near coords,
            nodes near coords align={vertical},
            nodes near coords style={font=\tiny},
            every node near coord/.append style={anchor=south},
        ]
        \addplot[color=pt1min,mark=square*] table[x=d,y=1]{\paramDPrec};
        \addplot[color=pt2min,mark=triangle*] table[x=d,y=2]{\paramDPrec};
        \addplot[color=pt4min,mark=otimes*] table[x=d,y=4]{\paramDPrec};
        \end{axis}
        \end{tikzpicture}
    }
    \resizebox{0.49\linewidth}{!}{
        \begin{tikzpicture}
        \begin{axis}[
            width=0.75\linewidth,
            ylabel={MAE (Coor, meters)},
            ymin=110, ymax=557,
            ytick distance={80},
            ymajorgrids=true,
            grid style=dashed,
            xtick=data,
            symbolic x coords={32,64,128,192,256},
            nodes near coords,
            nodes near coords align={vertical},
            nodes near coords style={font=\tiny},
            every node near coord/.append style={anchor=south},
        ]
        \addplot[color=pt1min,mark=square*] table[x=d,y=1]{\paramDMAE};
        \addplot[color=pt2min,mark=triangle*] table[x=d,y=2]{\paramDMAE};
        \addplot[color=pt4min,mark=otimes*] table[x=d,y=4]{\paramDMAE};
        \end{axis}
        \end{tikzpicture}
    }
    \label{fig:hyper-parameter-d}
}

\subfigure[Number of Attention heads $N_h$] {
    \resizebox{0.49\linewidth}{!}{
        \begin{tikzpicture}
        \begin{axis}[
            width=0.75\linewidth,
            ylabel={Precision (\%)},
            ymin=73, ymax=91,
            ytick distance={3},
            ymajorgrids=true,
            grid style=dashed,
            xtick=data,
            symbolic x coords={1,2,4,8,16},
            nodes near coords,
            nodes near coords align={vertical},
            nodes near coords style={font=\tiny},
            every node near coord/.append style={anchor=south},
        ]
        \addplot[color=pt1min,mark=square*] table[x=N_h,y=1]{\paramNhPrec};
        \addplot[color=pt2min,mark=triangle*] table[x=N_h,y=2]{\paramNhPrec};
        \addplot[color=pt4min,mark=otimes*] table[x=N_h,y=4]{\paramNhPrec};
        \end{axis}
        \end{tikzpicture}
    }
    \resizebox{0.49\linewidth}{!}{
        \begin{tikzpicture}
        \begin{axis}[
            width=0.75\linewidth,
            ylabel={MAE (Coor, meters)},
            ymin=110, ymax=557,
            ytick distance={80},
            ymajorgrids=true,
            grid style=dashed,
            xtick=data,
            xtick=data,
            symbolic x coords={1,2,4,8,16},
            nodes near coords,
            nodes near coords align={vertical},
            nodes near coords style={font=\tiny},
            every node near coord/.append style={anchor=south},
        ]
        \addplot[color=pt1min,mark=square*] table[x=N_h,y=1]{\paramNhMAE};
        \addplot[color=pt2min,mark=triangle*] table[x=N_h,y=2]{\paramNhMAE};
        \addplot[color=pt4min,mark=otimes*] table[x=N_h,y=4]{\paramNhMAE};
        \end{axis}
        \end{tikzpicture}
    }
    \label{fig:hyper-parameter-N_h}
}

\subfigure[Distance threshold $\delta$ (meters)] {
    \resizebox{0.49\linewidth}{!}{
        \begin{tikzpicture}
        \begin{axis}[
            width=0.75\linewidth,
            ylabel={Precision (\%)},
            ymin=73, ymax=91,
            ytick distance={3},
            ymajorgrids=true,
            grid style=dashed,
            xtick=data,
            symbolic x coords={10,50,100,150,200},
            nodes near coords,
            nodes near coords align={vertical},
            nodes near coords style={font=\tiny},
            every node near coord/.append style={anchor=south},
        ]
        \addplot[color=pt1min,mark=square*] table[x=delta,y=1]{\paramDeltaPrec};
        \addplot[color=pt2min,mark=triangle*] table[x=delta,y=2]{\paramDeltaPrec};
        \addplot[color=pt4min,mark=otimes*] table[x=delta,y=4]{\paramDeltaPrec};
        \end{axis}
        \end{tikzpicture}
    }
    \resizebox{0.49\linewidth}{!}{
        \begin{tikzpicture}
        \begin{axis}[
            width=0.75\linewidth,
            ylabel={MAE (Coor, meters)},
            ymin=110, ymax=557,
            ytick distance={80},
            ymajorgrids=true,
            grid style=dashed,
            xtick=data,
            symbolic x coords={10,50,100,150,200},
            nodes near coords,
            nodes near coords align={vertical},
            nodes near coords style={font=\tiny},
            every node near coord/.append style={anchor=south},
        ]
        \addplot[color=pt1min,mark=square*] table[x=delta,y=1]{\paramDeltaMAE};
        \addplot[color=pt2min,mark=triangle*] table[x=delta,y=2]{\paramDeltaMAE};
        \addplot[color=pt4min,mark=otimes*] table[x=delta,y=4]{\paramDeltaMAE};
        \end{axis}
        \end{tikzpicture}
    }
    \label{fig:hyper-parameter-delta}
}
